Radial BPZ equations and partition functions of FK-Ising interfaces conditional on one-arm event

Radial BPZ equations come naturally when one solves Dub\'{e}dat's commutation relation in the radial setting. We construct positive solutions to radial BPZ equations and show that partition functions of FK-Ising interfaces in a polygon conditional on a one-arm event are positive solutions to radial BPZ equations.

==> tex/multipleSLE_BPZ.tex <==
The goal of this section is to prove Proposition~\ref{prop::solutions_evenr2} and the following related property. 



\paragraph*{Radial Loewner chain.}
Suppose $K\subset\U$ is a compact set such that $\U\setminus K$ is simply connected and contains the origin. Let $\varphi$ be the conformal map from $\U\setminus K$ onto $\U$ with $\varphi(0)=0$ and $\varphi'(0)>0$. 
The \textit{capacity} of $K$ is $\log \varphi'(0)=-\log\CR(\U\setminus K)$. 
Fix $\theta\in [0,2\pi)$, suppose $\eta: [0,T]\to \overline{\U}$ is a continuous non-self-crossing curve such that $\eta_0=\exp(\ii\theta)$ and $\eta_{(0,T)}\subset\U$. Let $D_t$ be the connected component of $\U\setminus\eta_{[0,t]}$ containing the origin. Let $g_t: D_t\to \U$ be the unique conformal map with $g_t(0)=0$ and $g_t'(0)>0$. We say that the curve is parameterized by capacity if $g_t'(0)=\ee^t$. Then $g_t$ solves the radial Loewner evolution:
\begin{equation}\label{eqn::radialLoewner_def}
\partial_t g_t(z)=g_t(z)\frac{\ee^{\ii\xi_t}+g_t(z)}{\ee^{\ii\xi_t}-g_t(z)},\quad g_0(z)=z,
\end{equation}
where $(\xi_t, t\ge 0)$ is called the \textit{driving function} of $\eta$. \textit{Radial $\SLE_{\kappa}$} is the radial Loewner chain with driving function $\xi_t=\sqrt{\kappa}B_t$ where $(B_t, t\ge 0)$ is one-dimensional Brownian motion.


\begin{theorem}\label{thm::multipleSLE_CR}
Fix $\kappa\in (0,6]$ and $\mathfrak{r}<1-\kappa/8$. 
\begin{itemize}
\item The expectation in~\eqref{eqn::multipleSLE_CRpf_def} is finite and $\LZalphar$ in~\eqref{eqn::multipleSLE_CRpf_def} satisfies the following $2N$ radial BPZ equations: 
\begin{align}\label{eqn::radialBPZ}
\frac{\kappa}{2}\frac{\partial_{j}^2\LZ}{\LZ}+\sum_{i\neq j}\left(\cot((\theta_i-\theta_j)/2)\frac{\partial_i\LZ}{\LZ}-\frac{(6-\kappa)/(4\kappa)}{\sin^2((\theta_i-\theta_j)/2)}\right)=\frac{(6-\kappa)(\kappa-2)}{8\kappa}-\mathfrak{r},
\end{align}
for all $j\in\{1,\ldots, 2N\}$, 
where $\partial_i$ is the partial derivative with respect to $\theta_i$. 
\item  Denote by $\PP(\LZalphar)$
the law of global multiple $\SLE_{\kappa}\sim\PP_{\alpha}$ weighted by $\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}$. Then the law of $\eta_j$ under $\PP(\LZalphar)$ is the same as radial Loewner chain whose driving function is the solution to the following SDE, up to the first time that $\exp(\ii\theta_{j-1})$ or $\exp(\ii\theta_{j+1})$ is disconnected from the origin: 
\begin{equation}\label{eqn::CR_driving_intro}
\begin{cases}
\ud \xi_t=\sqrt{\kappa}\ud B_t+\kappa\partial_j(\log\LZalphar)(V_t^1, \ldots, V_t^{j-1}, \xi_t, V_t^{j+1}, \ldots, V_t^{2N})\ud t, \quad \xi_0=\theta_j;\\
\ud V_t^i=\cot\left((V_t^i-\xi_t)/2\right)\ud t, \quad V_0^i=\theta_i,\quad\text{for }i\in\{1,\ldots, j-1, j+1, \ldots, 2N\}.
\end{cases}
\end{equation}
\end{itemize}
\end{theorem}

The rest of this section is organized as follows. In Section~\ref{subsec::SLE_pre}, we collect some preliminary tools. In Section~\ref{subsec::multipleSLE_CR}, we prove Theorem~\ref{thm::multipleSLE_CR}. In Section~\ref{subsec::multipleSLE_CR_asy}, we derive asymptotic property of variants of partition functions $\LZalphar$. Sucn asymptotic property provides a tool to investigate the linear independence of solutions to radial BPZ equations~\eqref{eqn::radialBPZ}. We end this section with Remark~\ref{rem::solutionspace} which discusses the dimension of the solution space of radial BPZ equations~\eqref{eqn::radialBPZ}. 
\subsection{Preliminaries}
\label{subsec::SLE_pre}

\paragraph*{Poisson kernel.}
\textit{(Boundary) Poisson kernel} $H(\Omega; x, y)$ is defined for nice Dobrushin domain $(\Omega; x, y)$. When $\Omega=\HH$, we have
\begin{equation}\label{eqn::Poisson_def_H}
H(\HH; x,y)=|y-x|^{-2},\quad x,y\in\R. 
\end{equation}
For nice Dobrushin domain $(\Omega; x, y)$, we extend its definition via conformal covariance: 
\begin{equation}\label{eqn::Poisson_def_general}
H(\Omega; x, y)=|\varphi'(x)\varphi'(y)|H(\HH; \varphi(x), \varphi(y)), 
\end{equation}
where $\varphi$ is any conformal map from $\Omega\to \HH$.
When $\Omega=\U$, we have
\begin{equation}
H(\U; \exp(\ii\theta_1), \exp(\ii\theta_2))=\left(2\sin((\theta_2-\theta_1)/2)\right)^{-2}.
\end{equation}
Poisson kernel satisfies the following monotonicity.
Let $(\Omega; x, y)$ be a nice Dobrushin domain and let $U\subset\Omega$ be a subdomain that agrees with $\Omega$ in a neighborhood of the boundary arc $(yx)$. Then we have
\begin{equation}\label{eqn::Poisson_mono}
H(U; x, y)\le H(\Omega; x, y).
\end{equation}


\paragraph*{Chordal SLE and conformal radius.} 
\begin{lemma}\label{lem::CR_expectation}
Fix $\kappa\in (0,8)$ and $\theta_1<\theta_2<\theta_1+2\pi$ and denote $\theta=\theta_2-\theta_1\in (0,2\pi)$. Suppose $\eta$ is chordal $\SLE_{\kappa}$ in $\U$ from $\exp(\ii \theta_1)$ to $\exp(\ii\theta_2)$ and denote by $\E^{(\theta_1, \theta_2)}$ the expectation with respect to $\eta$. 
We denote by $\CR(\U\setminus\eta)$ the conformal radius of the connected component of $\U\setminus \eta$ containing the origin.  For $\mathfrak{r}\in \mathbb{R}$, 
we define 
\begin{align}\label{eqn::CR_expectation}
\begin{split}
\Phi^R(\kappa, \mathfrak{r}; u):=&\E^{(\theta_1, \theta_2)}\left[\one\{\text{origin is to the right of $\eta$}\}\CR(\U\setminus\eta)^{-\mathfrak{r}}\right],\\
\Phi^L(\kappa, \mathfrak{r}; u):=&\E^{(\theta_1, \theta_2)}\left[\one\{\text{origin is to the left of $\eta$}\}\CR(\U\setminus\eta)^{-\mathfrak{r}}\right],\\
\Phi(\kappa, \mathfrak{r}; u):=&\E^{(\theta_1, \theta_2)}\left[\CR(\U\setminus\eta)^{-\mathfrak{r}}\right],\qquad\text{where }u=\sin^2(\theta/4)\in (0,1).
\end{split}
\end{align}
Then $\Phi(\kappa, \mathfrak{r}; u)$ is finite for $u\in (0,1)$ if only and if $\mathfrak{r}<1-\kappa/8$. Moreover, when $\mathfrak{r}<1-\kappa/8$, $\Phi^L(\kappa, \mathfrak{r}; \cdot), \Phi^R(\kappa, \mathfrak{r}; \cdot)$ and $\Phi(\kappa, \mathfrak{r}; \cdot)$ all satisfy the following Euler's hypergeometric differential equation:
\begin{equation}\label{eqn::CR_ODE}
    u(1-u)\Phi''+\frac{3\kappa-8}{2\kappa}(1-2u)\Phi'+\frac{8\mathfrak{r}}{\kappa}\Phi=0.
\end{equation}
\end{lemma} 
\begin{proof}
See~\cite[Proof of Lemma~3.10]{WangWuCommutationRelation}. 
%In particular, when $\mathfrak{r}\in (0,1-\kappa/8)$, we define 
%\begin{equation*}
%    A=1-\frac{4}{\kappa}+\sqrt{\left(1-\frac{4}{\kappa}\right)^2+\frac{8\mathfrak{r}}{\kappa}}, \quad B=1-\frac{4}{\kappa}-\sqrt{\left(1-\frac{4}{\kappa}\right)^2+\frac{8\mathfrak{r}}{\kappa}},\quad C=\frac{3}{2}-\frac{4}{\kappa}.
%\end{equation*}
%Assume $C\not\in\mathbb{Z}$ and define 
%\begin{align*}
%    f_1(u):=\hF(A, B, C; u), \quad f_2(u):=u^{1-C}\hF(1+A-C, 1+B-C, 2-C, u),
%\end{align*}
%where $\hF$ is the hypergeometric function (see e.g.~\cite[Eq.(15.1.1)]{AbramowitzHandbook}). Note that $f_1, f_2$ are two linearly independent solutions to ODE~\eqref{eqn::CR_ODE} with boundary data
%\begin{align*}
%f_1(0)=&1,\quad f_1(1)=\frac{\Gamma(C)\Gamma(C-A-B)}{\Gamma(C-A)\Gamma(C-B)}=\frac{\cos\left(\pi\sqrt{\left(1-\frac{4}{\kappa}\right)^2+\frac{8\mathfrak{r}}{\kappa}}\right)}{\cos\left(\pi\left(1-\frac{4}{\kappa}\right)\right)};\\
%    f_2(0)=&0, \quad f_2(1)=\frac{\Gamma(2-C)\Gamma(1-C)}{\Gamma(1-A)\Gamma(1-B)}\in (0,\infty).
%\end{align*}
%From~\cite[Proof of Lemma~3.10]{WangWuCommutationRelation}, we have
%\begin{align}\label{eqn::CR_expectation_right_aux}
%\Phi^R(\kappa, \mathfrak{r}; u)=f_2(u)/f_2(1). 
%\end{align}
\end{proof}

Let us investigate the solution to~\eqref{eqn::CR_ODE} with $\mathfrak{r}=\mathfrak{r}_1(\kappa)$ which is one-arm exponent for conformal loop ensemble~\eqref{eqn::onearmexponent}: 
\begin{equation*}
\mathfrak{r}_1(\kappa)=\frac{(3\kappa-8)(8-\kappa)}{32\kappa}. 
\end{equation*}
By direct calculation, we find 
\[\phi(u)=u^{4/\kappa-1/2}\]
is a solution to~\eqref{eqn::CR_ODE} with $\mathfrak{r}=\mathfrak{r}_1(\kappa)$ and boundary data $\phi(0)=0$ and $\phi(1)=1$. Combining with Lemma~\ref{lem::CR_expectation}, we obtain the following conclusion.
\begin{corollary}\label{cor::CR_expectation_onearm}
Assume the same notations as in Lemma~\ref{lem::CR_expectation}. Then 
\begin{align}\label{eqn::CR_expectation_onearm}
\begin{split}
&\E^{(\theta_1, \theta_2)}\left[\one\{\text{origin is to the right of $\eta$}\}\CR(\U\setminus\eta)^{-\mathfrak{r}_1(\kappa)}\right]=\left(\sin(\theta/4)\right)^{8/\kappa-1};\\
&\E^{(\theta_1, \theta_2)}\left[\one\{\text{origin is to the left of $\eta$}\}\CR(\U\setminus\eta)^{-\mathfrak{r}_1(\kappa)}\right]=\left(\cos(\theta/4)\right)^{8/\kappa-1};\\
&\E^{(\theta_1, \theta_2)}\left[\CR(\U\setminus\eta)^{-\mathfrak{r}_1(\kappa)}\right]=\left(\sin(\theta/4)\right)^{8/\kappa-1}+\left(\cos(\theta/4)\right)^{8/\kappa-1}. 
\end{split}
\end{align}
\end{corollary}

We collect the following estimates which will be useful later.
\begin{corollary}\label{cor::CR_estimate}
Assume the same notations as in Lemma~\ref{lem::CR_expectation}.
For any $0<\mathfrak{r}<p< 1-\kappa/8$, we have
\begin{align}\label{eqn::CR_estimate1}
&\PP^{(\theta_1,\theta_2)}\left[\CR(\U\setminus\eta)\le \eps\right]
\le  \eps^{p}\Phi(\kappa, p;\sin^2(\t/4));\\
&\E^{(\theta_1,\theta_2)}\left[\one\{\CR(\U\setminus\eta)\le \eps\}\CR(\U\setminus\eta)^{-\mathfrak{r}}\right] \le  \eps^{p-r}\Phi(\kappa, p; \sin^2(\t/4)). \label{eqn::CR_estimate2}
\end{align}
\end{corollary}
\begin{proof}
We denote $u=\sin^2(\t/4)$. By Markov inequality, we have
\begin{align*}
\PP^{(\theta_1,\theta_2)}\left[\CR(\U\setminus\eta)\le \eps\right]=&\PP^{(\theta_1,\theta_2)}\left[\CR(\U\setminus\eta)^{-p}\ge \eps^{-p}\right]\\
\le& \eps^{p}\E^{(\theta_1,\theta_2)}\left[\CR(\U\setminus\eta)^{-p}\right]=\eps^{p}\Phi(\kappa, p;u).
\end{align*}
This completes the proof of~\eqref{eqn::CR_estimate1}. 

We pick $q>1$ such that $\mathfrak{r}/p+1/q=1$. From H\"{o}lder inequality, we have
\begin{align*}
\E^{(\theta_1,\theta_2)}\left[\one\{\CR(\U\setminus\eta)\le \eps\}\CR(\U\setminus\eta)^{-\mathfrak{r}}\right]
\le& \PP^{(\theta_1, \theta_2)}\left[\CR(\U\setminus\eta)
\le \eps\right]^{1/q}\E^{(\theta_1,\theta_2)}\left[\CR(\U\setminus\eta)^{-p}\right]^{\mathfrak{r}/p}\notag\\
=& \PP^{(\theta_1, \theta_2)}\left[\CR(\U\setminus\eta)
\le \eps\right]^{1/q}\Phi(\kappa, p; u)^{\mathfrak{r}/p}\\
\le &\eps^{p/q}\Phi(\kappa, p; u)^{1/q}\Phi(\kappa, p; u)^{\mathfrak{r}/p}=\eps^{p-\mathfrak{r}}\Phi(\kappa, p; u).
\end{align*}
This completes the proof of~\eqref{eqn::CR_estimate2}. 
\end{proof}



\subsection{Multiple SLEs and proof of Theorem~\ref{thm::multipleSLE_CR}}
\label{subsec::multipleSLE_CR}
We usually consider multiple SLEs and their corresponding pure partition functions in the upper-half plane $\HH$, see Appendix~\ref{appendix::chordalBPZ}. In this article, it is more convenient to work in the unit disc $\U$. As they are conformally invariant and conformally covariant respectively, transforming their properties from $\HH$ to $\U$ is just a change of variables. 

Fix parameters
\begin{equation}\label{eqn::htildeh_def}
\kappa\in (0,6],\qquad h=\frac{6-\kappa}{2\kappa},\qquad\tilde{h}=\frac{(6-\kappa)(\kappa-2)}{8\kappa}. 
\end{equation}
%Suppose $\{\LZ_{\alpha}(\Omega; x_1, \ldots, x_{2N}): \alpha\in\LP_N\}$ is the collection of pure partition functions for a nice polygon $(\Omega; x_1, \ldots, x_{2N})$ in Appendix~\ref{appendix::chordalBPZ}. We focus on $\Omega=\U$, for $\theta_1<\cdots<\theta_{2N}<\theta_1+2\pi$, we denote 
%\[\LZ_{\alpha}(\theta_1, \ldots, \theta_{2N})=\LZ_{\alpha}(\U; \exp(\ii\theta_1), \ldots, \exp(\ii\theta_{2N})).\]
%Then pure partition functions $\{\LZ_{\alpha}(\theta_1, \ldots, \theta_{2N}): \alpha\in\LP_N\}$ satisfy radial BPZ equations~\eqref{eqn::radialBPZ} with $\mathfrak{r}=0$.
We assume $\theta_1<\cdots<\theta_{2N}<\theta_1+2\pi$ and denote $x_j=\exp(\ii\theta_j)$ for $1\le j\le 2N$. 
For $\alpha\in\LP_N$, recall from~\eqref{eqn::multipleSLE_def} that $\PP_{\alpha}$ denotes the law of global multiple $\SLE_{\kappa}$ in $(\U; x_1, \ldots, x_{2N})$ associated to link pattern $\alpha$. We write $\alpha=\{\{a_1, b_1\}, \ldots, \{a_N, b_N\}\}\in\LP_N$ and we keep the ordering~\eqref{eqn::linkpattern_order}. 
The goal of this section is to derive in Proposition~\ref{prop::multipleSLE_CR_finite} a power law bound for $\LZalphar$ in~\eqref{eqn::multipleSLE_CRpf_def}  and then prove Theorem~\ref{thm::multipleSLE_CR}. 
\begin{proposition}\label{prop::multipleSLE_CR_finite}
Fix $\kappa\in (0,6]$ and denote $h=(6-\kappa)/(2\kappa)$ as in~\eqref{eqn::htildeh_def} and write $\alpha\in\LP_N$ as in~\eqref{eqn::linkpattern_order}. 
Suppose $(\eta_1, \ldots, \eta_N)\sim \PP_{\alpha}$, we denote by $\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)$ the conformal radius of the connected component of $\U\setminus\cup_{j=1}^N\eta_j$ containing the origin. For $\mathfrak{r}<1-\kappa/8$, 
the function $\LZalphar$ defined in~\eqref{eqn::multipleSLE_CRpf_def}
\[\LZ_{\alpha}^{(\mathfrak{r})}(\theta_1, \ldots, \theta_{2N})=\LZ_{\alpha}(\theta_1, \ldots, \theta_{2N})\E_{\alpha}\left[\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}\right]
\]
has the following upper bound: there exists a constant $C^{(\mathfrak{r})}\in(0,\infty)$ depending only on $\mathfrak{r}$ such that 
\begin{align}\label{eqn::multipleSLE_CRpf_upperbound}
\LZ_{\alpha}^{(\mathfrak{r})}(\theta_1, \ldots, \theta_{2N})\le NC^{(\mathfrak{r})}\prod_{s=1}^N \left(2\sin((\theta_{b_s}-\theta_{a_s})/2)\right)^{-2h}. 
\end{align}
\end{proposition}

To prove Proposition~\ref{prop::multipleSLE_CR_finite} and Theorem~\ref{thm::multipleSLE_CR}, we need the following two lemmas. 
In Lemma~\ref{lem::multipleSLEvsradialSLE}, 
We will compare the law of $\eta_1$ under $\PP_{\alpha}$ and the law of radial SLE. In Lemma~\ref{lem::multipleSLEvschordalSLE}, we will compare the law of $\eta_1$ under $\PP_{\alpha}$ and the law of chordal SLE. 

\begin{lemma}\label{lem::multipleSLEvsradialSLE}
Suppose $\eta: [0,T]\to \overline{\U}$ is a continuous non-self-crossing curve such that $\eta_0=\exp(\ii\theta_1)$. Let $g_t$ be the radial Loewner chain~\eqref{eqn::radialLoewner_def} and denote by $\phi_t$ the covering map of $g_t$, i.e. 
$g_t(\exp(\ii w))=\exp(\ii\phi_t(w))$ with $\phi_0(w)=w$ for $w\in\HH$. We denote $V_t^j=\phi_t(\theta_j)$ for $j=2,\ldots, 2N$
with $\xi_t<V_t^2<\cdots<V_t^{2N}$. 

Suppose $(\eta_1, \ldots, \eta_N)\sim\PP_{\alpha}$.
Then the law of $\eta_1$ under $\PP_{\alpha}$ is the same as radial $\SLE_{\kappa}$ in $(\U; \exp(\ii\theta_1); 0)$ weighted by the following local martingale, up to the first time $\exp(\ii\theta_{2N})$ or $\exp(\ii\theta_2)$ is disconnected from the origin:
\begin{equation}\label{eqn::mart_multipleSLE}
M_t(\LZ_{\alpha})=g_t'(0)^{-\tilde{h}}\times\prod_{j=2}^{2N}\phi_t'(\theta_j)^h\times\LZ_{\alpha}(\xi_t, V_t^2, \ldots, V_t^{2N}). 
\end{equation}  
\end{lemma}
\begin{proof}
Analogous conclusion is known for the upper-half plane, see~\cite[Section~6]{WuHyperSLE}. From $\HH$ to $\U$, we perform a standard change of variables calculation~\cite{SchrammWilsonSLECoordinatechanges}. 
\end{proof}

Recall that $\eta_1$ under $\PP_{\alpha}$ is a curve in $\U$ from $x_{a_1}$ to $x_{b_1}$. We will introduce the Radon-Nikodym derivative between $\eta_1$ under $\PP_{\alpha}$ and chordal $\SLE_{\kappa}$ in $(\U; x_{a_1}, x_{b_1})$ below. 
For $\alpha=\{\{a_1, b_1\}, \ldots, \{a_N, b_N\}\}$, the link $\{a_1, b_1\}$ divides $\alpha$ into two sub-link patterns, connecting $\{a_1+1, \ldots, b_1-1\}$ and $\{b_1+1, \ldots, a_1-1\}$ respectively. After relabeling the indices, we denote these two link patterns by $\alpha_1^R$ and $\alpha_1^L$. 
Suppose $\eta$ is $\SLE_{\kappa}$ in $\U$ from $x_{a_1}$ to $x_{b_1}$, we say that $\eta$ is allowed by $\alpha$ if, for all $s\neq 1$, the points $x_{a_s}$ and $x_{b_s}$ lie on the boundary of the same connected component of $\U\setminus\eta$. In other words, $\eta$ is allowed by $\alpha$ if it does not disconnect any pair of points $\{x_{a_s}, x_{b_s}\}$ for $s\neq 1$. We denote this event by $\LE_{\alpha}(\eta)$. On the event $\LE_{\alpha}(\eta)$, the points $x_{a_1+1}, \ldots, x_{b_1-1}$ are divided into smaller groups. We denote the connected components of $\U\setminus\eta$ having these points on the boundary by $U_1^{R, 1}, \ldots, U_1^{R, r}$ in counterclockwise order and denote their union by $U_1^R$. The sub-link pattern $\alpha_1^R$ is further divided into smaller sub-link patterns, after relabeling the indices, we denote these link patterns by $\alpha_1^{R, 1}, \ldots, \alpha_1^{R, r}$. We define 
\[\LZ_{\alpha_1^R}(U^R_1; x_{a_1+1}, \ldots, x_{b_1-1})=\LZ_{\alpha_1^{R,1}}(U_1^{R,1}; \ldots)\times\cdots\times\LZ_{\alpha_1^{R, r}}(U_1^{R, r}; \ldots).\]
We define $U_1^{L, 1}, \ldots, U_1^{L, \ell}, U_1^L, \alpha_1^{L, 1}, \ldots, \alpha_1^{L,\ell}$ similarly and define 
\[\LZ_{\alpha_1^L}(U^L_1; x_{b_1+1}, \ldots, x_{a_1-1})=\LZ_{\alpha_1^{L,1}}(U_1^{L,1}; \ldots)\times\cdots\times\LZ_{\alpha_1^{L, \ell}}(U_1^{L, \ell}; \ldots).\]
We also write 
\begin{align*}
&\LZ_{\alpha/\{a_1, b_1\}}(\U\setminus\eta; x_{a_1+1}, \ldots, x_{b_1-1}, x_{b_1+1}, \ldots, x_{a_1-1})\\
=&\LZ_{\alpha_1^R}(U^R_1; x_{a_1+1}, \ldots, x_{b_1-1})\times \LZ_{\alpha_1^L}(U^L_1; x_{b_1+1}, \ldots, x_{a_1-1}).
\end{align*}
\begin{lemma}\label{lem::multipleSLEvschordalSLE}
\cite[Section~6]{WuHyperSLE}.
The law of $\eta_1$ under $\PP_{\alpha}$ is the same as $\eta\sim$ chordal $\SLE_{\kappa}$ in $(\U; x_{a_1}, x_{b_1})$ weighted by 
\[\frac{\LZtwo(\U; x_{a_1}, x_{b_1}) }{\LZ_{\alpha}(\U; x_1, \ldots, x_{2N})}\LZ_{\alpha/\{a_1, b_1\}}(\U\setminus\eta; x_{a_1+1}, \ldots, x_{b_1-1}, x_{b_1+1}, \ldots, x_{a_1-1})\one\{\LE_{\alpha}(\eta)\}.\]
\end{lemma}

\begin{proof}[Proof of Proposition~\ref{prop::multipleSLE_CR_finite}]
Note that the conformal radius $\CR(\U\setminus\cup_{j=1}^N\eta_j)\le 1$. If $\mathfrak{r}\le 0$, from~\eqref{eqn::PPF_bound_polygon}, we have
\[\LZ_{\alpha}^{(\mathfrak{r})}(\theta_1, \ldots, \theta_{2N})\le \LZ_{\alpha}(\theta_1, \ldots, \theta_{2N})\le \prod_{s=1}^N \left(2\sin((\theta_{b_s}-\theta_{a_s})/2)\right)^{-2h},
\]
as desired in~\eqref{eqn::multipleSLE_CRpf_upperbound}. In the rest of the proof, we assume $\mathfrak{r}>0$.

We write $\alpha\in\LP_N$ as in~\eqref{eqn::linkpattern_order}. 
Let us estimate the probability \[
\PP_{\alpha}\left[\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)\le \eps\right]\] for $\eps>0$ small. 
For any subset $K\subset\U$, Koebe's one quarter theorem gives 
$\dist(0,K)\le \CR(\U\setminus K)\le 4\dist(0,K)$.
Thus,
\begin{align*}
\left\{\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)\le \eps\right\}
\quad \subset\quad 
\cup_{j=1}^N\left\{\dist(0,\eta_j)\le \eps\right\}
\quad \subset\quad
\cup_{j=1}^N\left\{\CR(\U\setminus\eta_j)\le 4\eps\right\}. 
\end{align*}
Consequently,
\begin{align}\label{eqn::multipleSLE_CR_aux2}
\PP_{\alpha}\left[\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)\le \eps\right]\le \sum_{j=1}^N\PP_{\alpha}\left[\CR(\U\setminus\eta_j)\le 4\eps\right].
\end{align}
It remains to estimate $\PP_{\alpha}[\CR(\U\setminus\eta_j)\le 4\eps]$.  

From Lemma~\ref{lem::multipleSLEvschordalSLE}, the law of $\eta_j$ under $\PP_{\alpha}$ is absolutely continuous with respect to $\eta\sim$ chordal $\SLE_{\kappa}$ in $(\U; x_{a_j}, x_{b_j})$. We denote by $\LE^j_{\alpha}(\eta)$ the event that $\eta$ is allowed by $\alpha$. Then the law of $\eta_j$ under $\PP_{\alpha}$ is the same as $\eta$ weighted by 
\[\frac{\LZtwo(\U; x_{a_j}, x_{b_j}) }{\LZ_{\alpha}(\U; x_1, \ldots, x_{2N})}\LZ_{\alpha_j^R}(U^R_j; x_{a_j+1}, \ldots, x_{b_j-1})\times \LZ_{\alpha_j^L}(U^L_j; x_{b_j+1}, \ldots, x_{a_j-1})\one\left\{\LE^j_{\alpha}(\eta)\right\}.\]
From~\eqref{eqn::PPF_bound_polygon} and the monotonicity of Poisson kernel~\eqref{eqn::Poisson_mono}, we have  
\begin{align}\label{eqn::multipleSLE_CR_aux1}
&\LZ_{\alpha_j^R}(U^R_j; x_{a_j+1}, \ldots, x_{b_j-1})\times \LZ_{\alpha_j^L}(U^L_j; x_{b_j+1}, \ldots, x_{a_j-1})
\le  \prod_{s\neq j}\left(2\sin((\theta_{b_s}-\theta_{a_s})/2)\right)^{-2h}. 
\end{align}
We pick $p\in (0,1-\kappa/8)$, then 
\begin{align*}
&\PP_{\alpha}[\CR(\U\setminus\eta_j)\le 4\eps]\\
=&\frac{\LZ_{\includegraphics[scale=0.2]{figures/link-0}}(\U; x_{a_j}, x_{b_j}) }{\LZ_{\alpha}(\U; x_1, \ldots, x_{2N})}\\
&\times\E^{(\theta_{a_j}, \theta_{b_j})}\left[\LZ_{\alpha_j^R}(U^R_j; x_{a_j+1}, \ldots, x_{b_j-1})\times \LZ_{\alpha_j^L}(U^L_j; x_{b_j+1}, \ldots, x_{a_j-1})\one\left\{\LE_{\alpha}^j(\eta)\cap\{\CR(\U\setminus\eta)\le 4\eps\}\right\}\right]\\
\le &\frac{\prod_{s=1}^N \left(2\sin((\theta_{b_s}-\theta_{a_s})/2)\right)^{-2h}}{\LZ_{\alpha}(\U; x_1, \ldots, x_{2N})}\PP^{(\theta_{a_j}, \theta_{b_j})}[\CR(\U\setminus\eta)\le 4\eps]\\
\le & \frac{\prod_{s=1}^N \left(2\sin((\theta_{b_s}-\theta_{a_s})/2)\right)^{-2h}}{\LZ_{\alpha}(\U; x_1, \ldots, x_{2N})}\Phi(\kappa, p; \sin^2((\theta_{b_j}-\theta_{a_j})/4))(4\eps)^p
\end{align*}
where we use~\eqref{eqn::multipleSLE_CR_aux1} to get the first  inequality and we use~\eqref{eqn::CR_estimate1} to get the second inequality. Combining this estimate with~\eqref{eqn::multipleSLE_CR_aux2}, we obtain:
\begin{align}\label{eqn::multipleSLE_CR_aux0}
\PP_{\alpha}\left[\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)\le \eps\right]\le 4^p\frac{F_{\alpha; p}(\theta_1, \ldots,\theta_{2N})}{\LZ_{\alpha}(\theta_1, \ldots, \theta_{2N})}\eps^p,
\end{align}
where 
\begin{align*}
F_{\alpha; p}(\theta_1, \ldots, \theta_{2N}):=\prod_{s=1}^N\left(2\sin((\theta_{b_s}-\theta_{a_s})/2)\right)^{-2h}\times \sum_{j=1}^N\Phi(\kappa, p; \sin^2((\theta_{b_j}-\theta_{a_j})/4)).
\end{align*}

With~\eqref{eqn::multipleSLE_CR_aux0} at hand, we are ready to show the conclusion. For $\mathfrak{r}\in (0, 1-\kappa/8)$, we pick $p\in (\mathfrak{r}, 1-\kappa/8)$, then we have
\begin{align*}
\E_{\alpha}\left[\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}\right]\le &\sum_{k=1}^{\infty}2^{k\mathfrak{r}}\PP_{\alpha}\left[2^{-k}\le \CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)\le 2^{-k+1}\right]\\
\le & 4^p\frac{F_{\alpha; p}(\theta_1, \ldots,\theta_{2N})}{\LZ_{\alpha}(\theta_1, \ldots, \theta_{2N})}\sum_{k=1}^{\infty}2^{k\mathfrak{r}}2^{-(k-1)p}\\
=&\frac{2^{2p+1}}{1-2^{\mathfrak{r}-p}}\frac{F_{\alpha; p}(\theta_1, \ldots,\theta_{2N})}{\LZ_{\alpha}(\theta_1, \ldots, \theta_{2N})}.
\end{align*}
Therefore, 
\begin{align*}
\LZalphar(\theta_1, \ldots, \theta_{2N})\le \frac{2^{2p+1}}{1-2^{\mathfrak{r}-p}}F_{\alpha; p}(\theta_1, \ldots,\theta_{2N}).
\end{align*}
Note that
$\Phi(\kappa, p;u)\le \Phi(\kappa, p;1/2)$ for all $u\in (0,1)$.
Thus,
\begin{align*}
\LZalphar(\theta_1, \ldots, \theta_{2N})\le \frac{2^{2p+1}}{1-2^{\mathfrak{r}-p}}N\Phi(\kappa, p; 1/2)\prod_{s=1}^N \left(2\sin((\theta_{b_s}-\theta_{a_s})/2)\right)^{-2h}.
\end{align*}
This gives~\eqref{eqn::multipleSLE_CRpf_upperbound} with the constant 
\[C^{(\mathfrak{r})}=\frac{2^{2p+1}}{1-2^{\mathfrak{r}-p}}\Phi(\kappa, p; 1/2),\]
by choosing some $p\in (\mathfrak{r}, 1-\kappa/8)$. 
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm::multipleSLE_CR}]
Suppose $(\eta_1, \ldots, \eta_N)\sim \PP_{\alpha}$, we denote by $\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)$ the conformal radius of the connected component of $\U\setminus\cup_{j=1}^N\eta_j$ containing the origin.
For $\mathrm{r}<1-\kappa/8$, the expectation in~\eqref{eqn::multipleSLE_CRpf_def} is finite due to Proposition~\ref{prop::multipleSLE_CR_finite}. We denote by 
$\PP(\LZalphar)$ the law of $\PP_{\alpha}$ weighted by $\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}$. 
It remains to show that $\LZalphar$ satisfies radial BPZ equations~\eqref{eqn::radialBPZ} and the law of $\eta_j$ under $\PP(\LZalphar)$ satisfies~\eqref{eqn::CR_driving_intro}. From the rotation symmetry, it suffices to show~\eqref{eqn::radialBPZ} and~\eqref{eqn::CR_driving_intro} for $j=1$. 

For $\eta=\eta_1$, let us calculate the conditional expectation of $\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}$ given $\eta_{[0,t]}$ for $t>0$ small. From the conformal invariance and domain Markov property of multiple SLE, we have
\begin{align}\label{eqn::mart_multipleSLE_aux1}
\E_{\alpha}\left[\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}\cond \eta_{[0,t]}\right]=\ee^{\mathfrak{r}t}\frac{\LZalphar(\xi_t, V_t^2, \ldots, V_t^{2N})}{\LZ_{\alpha}(\xi_t, V_t^2, \ldots, V_t^{2N})}=\frac{M_t(\LZalphar)}{M_t(\LZ_{\alpha})}, 
\end{align}
where $M_t(\LZ_{\alpha})$ is defined in~\eqref{eqn::mart_multipleSLE} and $M_t(\LZalphar)$ is defined analogously :
\begin{equation}\label{eqn::mart_multipleSLE_CR}
M_t(\LZalphar)=g_t'(0)^{\mathfrak{r}-\tilde{h}}\times\prod_{j=2}^{2N}\phi_t'(\theta_j)^h\times\LZalphar(\xi_t, V_t^2, \ldots, V_t^{2N}). 
\end{equation}  
Combining Lemma~\ref{lem::multipleSLEvsradialSLE} and~\eqref{eqn::mart_multipleSLE_aux1}, the law of $\eta=\eta_1$ under $\PP(\LZalphar)$ is the same as radial $\SLE_{\kappa}$ in $(\U; \exp(\ii\theta_1); 0)$ weighted by $M_t(\LZalphar)$. 

Let us calculate $\ud M_t(\LZalphar)$ assuming that $\LZalphar$ is $C^2$. Recall that
\begin{align*}
g_t(0)=0, \quad g_t'(0)=\ee^t,\quad &\partial_t \phi_t(w)=\cot((\phi_t(w)-\xi_t)/2),\quad 
\partial_t\phi_t'(w)=-\frac{1}{2}\csc^2((\phi_t(w)-\xi_t)/2)\phi_t'(w). 
\end{align*}
Thus, 
\begin{align*}
&\frac{\ud M_t(\LZalphar)}{M_t(\LZalphar)}\\
=&(\mathfrak{r}-\tilde{h})\ud t+\sum_{j=2}^{2N}(-\frac{h}{2})\csc^2\left((V_t^j-\xi_t)/2\right)\ud t+\frac{\partial_1\LZalphar}{\LZalphar}\ud \xi_t+\sum_{j=2}^{2N}\frac{\partial_j\LZalphar}{\LZalphar}\cot\left((V_t^j-\xi_t)/2\right)\ud t+\frac{\kappa}{2}\frac{\partial_1^2\LZalphar}{\LZalphar}\ud t\\
=&\frac{\partial_1\LZalphar}{\LZalphar}\ud \xi_t+\left[\frac{\kappa}{2}\frac{\partial_1^2\LZalphar}{\LZalphar}+\sum_{j=2}^{2N}\left(\cot\left((V_t^j-\xi_t)/2\right)\frac{\partial_j\LZalphar}{\LZalphar}-\frac{h}{2}\csc^2\left((V_t^j-\xi_t)/2\right)\right)+(\mathfrak{r}-\tilde{h})\right]\ud t.
\end{align*}


As $M_t(\LZalphar)$ is a local martingale for radial $\SLE_{\kappa}$, the function $\LZalphar$ has to solve radial BPZ equation~\eqref{eqn::radialBPZ} with $j=1$ under the assumption that $\LZalphar$ is $C^2$. Let us elaborate the $C^2$ assumption here. In fact, the above analysis implies that $\LZalphar$ is a weak solution for~\eqref{eqn::radialBPZ} with $j=1$ (see~\cite[Appendix~A]{FengLiuPeltolaWu2024}). As the operator in~\eqref{eqn::radialBPZ} is hypoelliptic, weak solutions are strong solutions, thus $\LZalphar$ is indeed smooth and satisfies~\eqref{eqn::radialBPZ} as desired. 

Finally, let us derive~\eqref{eqn::CR_driving_intro} with $j=1$. From the above analysis, the law of $\eta=\eta_1$ under $\PP(\LZalphar)$ is the same as radial $\SLE_{\kappa}$ weighted by the local martingale $M_t(\LZalphar)$, this gives~\eqref{eqn::CR_driving_intro} and completes the proof. 
\end{proof}

From the conformal covariance of pure partition functions and conformal invariance of global multiple SLEs, we may extend the definition of $\LZalphar$ to a nice polygon with an interior point $(\Omega; x_1, \ldots, x_{2N}; z)$ via conformal covariance: for any conformal map $\varphi$ from $\Omega$ onto $\U$ such that $\varphi(z)=0$, 
\begin{equation}\label{eqn::multipleSLE_CRpf_cov}
\LZalphar(\Omega; x_1, \ldots, x_{2N}; z)=\prod_{j=1}^{2N}|\varphi'(x_j)|^h\times|\varphi'(z)|^\mathfrak{r}\times\LZalphar(\theta_1, \ldots, \theta_{2N}),
\end{equation}
where $\exp(\ii\theta_j)=\varphi(x_j)$ with $\theta_1<\cdots<\theta_{2N}<\theta_1+2\pi$. The upper bound~\eqref{eqn::multipleSLE_CRpf_upperbound} can be extended as follows:
\begin{equation}\label{eqn::multipleSLE_CRpf_upperbound_polygon}
\LZalphar(\Omega; x_1, \ldots, x_{2N}; z)\le NC^{(\mathfrak{r})}|\varphi'(z)|^{\mathfrak{r}}\prod_{\{a,b\}\in\alpha}H(\Omega; x_a, x_b)^{h}. 
\end{equation}


\subsection{Asymptotic properties}
\label{subsec::multipleSLE_CR_asy}
Let us investigate more about the expectation of the conformal radius. Suppose $(\eta_1, \ldots, \eta_N)\sim\PP_{\alpha}$ and we write $\alpha\in\LP_N$ as in~\eqref{eqn::linkpattern_order}. Suppose $\eta_j$ is a curve in $\U$ from $x_{a_j}$ to $x_{b_j}$. When $\kappa\le 4$, these curves are simple and $\U\setminus\cup_{j=1}^N\eta_j$ has $N+1$ connected components, we denote these connected components by $\LC_1, \ldots, \LC_{N+1}$ so that $\LC_j$ is the connected component stays to the right of $\eta_j$ for $1\le j\le N$ and $\LC_{N+1}$ is the last connected component which is the connected component stays to the left of $\eta_1$, see Figure~\ref{fig::twosle}. 
For $\kappa>4$, the curves have self-touching and $\U\setminus\cup_{j=1}^N\eta_j$ has countably many connected components. We define $\LC_1, \ldots, \LC_{N+1}$ analogously: for $1\le j\le N$, let $\LC_j$ be the union of the connected components which are to the right of $\eta_j$ but are not to the right of other $\eta_s$ for $s\neq j$, and let $\LC_{N+1}$ be the union of the connected components which are to the left of $\eta_1$ but are not to the right of other $\eta_s$ for $s\neq 1$. 
For $n\in\{1, \ldots, N+1\}$, define 
\begin{equation}\label{eqn::multipleSLE_CR_pf_more}
\LZalpharn(\theta_1, \ldots, \theta_{2N})=\LZ_{\alpha}(\theta_1, \ldots, \theta_{2N})\E_{\alpha}\left[\one\{0\in\LC_{n}\}\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}\right].
\end{equation}
Note that 
\[\LZalphar(\theta_1, \ldots, \theta_{2N})=\sum_{n=1}^{N+1}\LZalpharn(\theta_1, \ldots, \theta_{2N}).\]
We may also extend the definition of $\LZalpharn$ to nice polygon with an interior point via conformal covariance~\eqref{eqn::multipleSLE_CRpf_cov}. 
\begin{figure}[ht!]
\includegraphics[width=0.4\textwidth]{figures/twosle1234.pdf}
\qquad
\includegraphics[width=0.4\textwidth]{figures/twosle1423.pdf}
\caption{\label{fig::twosle}}
\end{figure}


When $N=1$, we have 
\begin{align*}
\LZtwoone^{(\mathfrak{r})}(\theta_1, \theta_2)=\LZtwo(\theta_1, \theta_2)\Phi^R(\kappa, \mathfrak{r}; \sin^2((\theta_2-\theta_1)/4));\\
\LZtwotwo^{(\mathfrak{r})}(\theta_1, \theta_2)=\LZtwo(\theta_1, \theta_2)\Phi^L(\kappa, \mathfrak{r}; \sin^2((\theta_2-\theta_1)/4));
\end{align*}
where $\Phi^R$ and $\Phi^L$ are defined in Lemma~\ref{lem::CR_expectation}. Both $\LZtwoone$ and $\LZtwotwo$ satisfy radial BPZ equations~\eqref{eqn::radialBPZ} with $N=1$, but they have different asymptotic behaviors when $\theta_2-\theta_1\to 0$. 
In the following proposition, we derive the asymptotic behavior of $\LZalpharn$. 
We assume $\theta_1<\cdots<\theta_{2N}<\theta_1+2\pi$ and denote $x_j=\exp(\ii\theta_j)$ for $1\le j\le 2N$. 


\begin{proposition}\label{prop::multipleSLE_CRpf_asy}
Fix $\kappa\in (0,6]$ and denote $h=(6-\kappa)/(2\kappa)$ as in~\eqref{eqn::htildeh_def}. 
The functions~\eqref{eqn::multipleSLE_CR_pf_more} all satisfy radial BPZ equations~\eqref{eqn::radialBPZ} and they have the following asymptotic properties. Fix $N\ge 1$ and $j\in\{1, \ldots, 2N-1\}$ and $n\in\{1, \ldots, N+1\}$. 
\begin{itemize}
\item If $\{j,j+1\}\in\alpha$, suppose $a_s=j$ and $b_s=j+1$, for all $\vartheta\in (\theta_{j-1}, \theta_{j+2})$, 
\begin{align}\label{eqn::multipleSLE_CR_pf_asypaired}
\lim_{\theta_j, \theta_{j+1}\to \vartheta}\frac{\LZalpharn(\theta_1, \ldots, \theta_{2N})}{(\theta_{j+1}-\theta_j)^{-2h}}=\begin{cases}
0,&\text{if }n=s;\\
\LZ_{\alpha/\{j,j+1\}; n}^{(\mathfrak{r})}(\theta_1, \ldots, \theta_{j-1}, \theta_{j+2}, \ldots, \theta_{2N}),&\text{if }n<s;\\
\LZ_{\alpha/\{j,j+1\}; n-1}^{(\mathfrak{r})}(\theta_1, \ldots, \theta_{j-1}, \theta_{j+2}, \ldots, \theta_{2N}),&\text{if }n>s;
\end{cases}
\end{align}
where $\alpha/\{j,j+1\}\in\LP_{N-1}$ denotes the link pattern obtained from $\alpha$ by removing the link $\{j,j+1\}$ and relabeling the remaining indices by $1,2\ldots, 2N-2$. 
\item If $\{j,j+1\}\not\in\alpha$, for all $\vartheta\in (\theta_{j-1}, \theta_{j+2})$, 
\begin{align}\label{eqn::multipleSLE_CR_pf_asynotpaired}
\lim_{\theta_j, \theta_{j+1}\to \vartheta}\frac{\LZalpharn(\theta_1, \ldots, \theta_{2N})}{(\theta_{j+1}-\theta_j)^{-2h}}=0.
\end{align}
\end{itemize}
\end{proposition}
\begin{proof}
Using a similar proof of Theorem~\ref{thm::multipleSLE_CR}, the functions~\eqref{eqn::multipleSLE_CR_pf_more} all satisfy radial BPZ equations~\eqref{eqn::radialBPZ}.
From the rotation symmetry of $\LZalpharn$, we only need to show the conclusion with $j=1$. The proof is split into Lemmas~\ref{lem::asy_paired_vanish}-\ref{lem::asy_notpaired_right}. 
\end{proof}

\begin{lemma}\label{lem::asy_paired_vanish}
The asymptotic in~\eqref{eqn::multipleSLE_CR_pf_asypaired} with $j=1$ and $n=1$ holds. 
\end{lemma}
\begin{proof}
In this case, we have $a_1=1$ and $b_1=2$.
We calculate the expectation conditional on $\eta_1$: 
\begin{align*}
\E_{\alpha}\left[\one\{0\in\LC_{1}\}\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}\cond \eta_1\right]=
\one\{0\in\LC_{1}\}\CR(\U\setminus\eta_1)^{-\mathfrak{r}}. 
\end{align*}
From Lemma~\ref{lem::multipleSLEvschordalSLE}, the law of $\eta_1$ under $\PP_{\alpha}$ is the same as $\eta\sim$ chordal $\SLE_{\kappa}$ in $(\U; x_1, x_2)$ weighted by
\begin{equation}\label{eqn::eta1vsetaRN}
\frac{\LZtwo(\U; x_1, x_2){\LZ_{\alpha/\{1,2\}}(\U\setminus \eta; x_3, \ldots, x_{2N})}}{\LZ_{\alpha}(\U; x_1, \ldots, x_{2N})}\one\{\LE_{\alpha}(\eta)\}.
\end{equation} 
Combining these two observations, we have
 \begin{align*}
 \frac{\LZalpharn(\U; x_1, \ldots, x_{2N};0)}{\LZtwo(\U; x_1, x_2)}=&\E^{(\theta_1, \theta_2)}\left[\one\{0\in\LC_{1}\}\CR(\U\setminus\eta)^{-\mathfrak{r}}\LZ_{\alpha/\{1,2\}}(\U\setminus \eta; x_3, \ldots, x_{2N})\one\{\LE_{\alpha}(\eta)\right]\\
 \le & \prod_{k=2}^N H(\U; x_{a_k}, x_{b_k})^h\times \E^{(\theta_1, \theta_2)}\left[\one\{0\in\LC_{1}\}\CR(\U\setminus\eta)^{-\mathfrak{r}}\right]\\
 =&\prod_{k=2}^N H(\U; x_{a_k}, x_{b_k})^h\times \Phi^R(\kappa, \mathfrak{r}; \sin^2((\theta_{2}-\theta_1)/4))\to 0,\quad\text{as }\theta_1, \theta_2\to \vartheta;
\end{align*}
where we use~\eqref{eqn::PPF_bound_polygon} and~\eqref{eqn::Poisson_mono} to get the inequality and we use Lemma~\ref{lem::CR_expectation} to get the second equality. This completes the proof of~\eqref{eqn::multipleSLE_CR_pf_asypaired} with $j=1$ and $n=1$. 
\end{proof}

\begin{lemma}\label{lem::asy_paired}
The asymptotic in~\eqref{eqn::multipleSLE_CR_pf_asypaired} with $j=1$ and $n>1$ holds. 
\end{lemma}
\begin{proof}
In this case, we have $a_1=1, b_1=2$. 
We calculate the expectation conditional on $\eta_1$: 
\begin{align}\label{eqn::asy_paired_aux1}
\E_{\alpha}\left[\one\{0\in\LC_{n}\}\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}\cond \eta_1\right]=\frac{\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta_1; x_3, \ldots, x_{2N}; 0)}{\LZ_{\alpha/\{1,2\}}(\U\setminus \eta_1; x_3, \ldots, x_{2N})}.
\end{align}
The function $\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta_1; x_3, \ldots, x_{2N}; 0)$ is understood in the following way. If $\kappa\le 4$, then $\U\setminus\eta_1$ has exactly two connected components, we denote by $U_1^L$ the one which has $x_3, \ldots, x_{2N}$ on the boundary. In this case, 
\[\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta_1; x_3, \ldots, x_{2N}; 0)=\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(U_1^L; x_3, \ldots, x_{2N}; 0)\]
If $\kappa\in (4,6]$, then $\U\setminus\eta_1$ has countably many connected components, we denote by $U_1^L, U_1^{L, 1}, \ldots, U_1^{L, \ell}$ as in Lemma~\ref{lem::multipleSLEvschordalSLE}. Let us consider the location of the origin. If the origin is contained in $U_1^L$, suppose $0\in U_1^{L, s}$, 
then $\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta_1; x_3, \ldots, x_{2N}; 0)$ is the product of partition functions of smaller domains 
\[\LZ_{\alpha_1^{L, 1}}(U_1^{L, 1}; \ldots)\times\cdots\times\LZ_{\alpha_1^{L, s-1}}(U_1^{L, s-1}; \ldots)\times\LZ_{\alpha_1^{L, s}}^{(\mathfrak{r})}(U_1^{L, s}; \ldots)\times\LZ_{\alpha_1^{L, s+1}}(U_1^{L, s+1}; \ldots)\times\cdots\times\LZ_{\alpha_1^{L, \ell}}(U_1^{L, \ell}; \ldots).\]
It is also possible that $0\not\in U_1^L$. In this case, denote by $\tilde{U}_1$ the connected component of $\U\setminus\eta_1$ containing the origin and set 
\[\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta_1; x_3, \ldots, x_{2N}; 0)=\CR(\tilde{U}_1)^{-\mathfrak{r}}\LZ_{\alpha/\{1,2\}}(U_1^L; x_3, \ldots, x_{2N}; 0).\]
 

Combining~\eqref{eqn::asy_paired_aux1} and~\eqref{eqn::eta1vsetaRN}, we have
\begin{align*}
\LZalpharn(\U; x_1, \ldots, x_{2N}; 0)=\LZtwo(\U; x_1, x_2)\E^{(\theta_1, \theta_2)}\left[\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta; x_3, \ldots, x_{2N}; 0)\right].
\end{align*}
To derive the conclusion, it suffices to show 
\begin{align}\label{eqn::asy_paired_aux2}
\lim_{\theta_1, \theta_2\to \vartheta}\E^{(\theta_1, \theta_2)}\left[\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta; x_3, \ldots, x_{2N}; 0)\right]
=\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U; x_3, \ldots, x_{2N}; 0). 
\end{align}

From~\eqref{eqn::multipleSLE_CRpf_upperbound_polygon} and~\eqref{eqn::Poisson_mono}, we have 
\begin{align*}
\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta; x_3, \ldots, x_{2N};0)\le N C^{(\mathfrak{r})}\CR(\U\setminus\eta)^{-\mathfrak{r}}\prod_{k=2}^N H(\U; x_{a_k}, x_{b_k})^h.
\end{align*}
If $\mathfrak{r}\le 0$, then bounded convergence theorem gives~\eqref{eqn::asy_paired_aux2}. In the following, we assume $\mathfrak{r}\in (0,1-\kappa/8)$. 
\begin{itemize}
\item On the one hand, $\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta; x_3, \ldots, x_{2N};0)$ is bounded on the event $\{\CR(\U\setminus\eta)\ge \eps\}$ for $\eps>0$. Thus, bounded convergence theorem guarantees
\begin{align*}%\label{eqn::asy_paired_aux3}
&\lim_{\theta_1, \theta_2\to \vartheta}\E^{(\theta_1, \theta_2)}\left[\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta; x_3, \ldots, x_{2N}; 0)\one\{\CR(\U\setminus\eta)\ge \eps\}\right]
\notag\\
=&\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U; x_3, \ldots, x_{2N}; 0). 
\end{align*}
\item On the other hand, 
\begin{align*}%\label{eqn::asy_paired_aux4}
&\E^{(\theta_1, \theta_2)}\left[\LZ_{\alpha/\{1,2\}; n-1}^{(\mathfrak{r})}(\U\setminus\eta; x_3, \ldots, x_{2N}; 0)\one\{\CR(\U\setminus\eta)\le \eps\}\right]\notag\\
\le & N C^{(\mathfrak{r})}\prod_{k=2}^N H(\U; x_{a_k}, x_{b_k})^h\E^{(\theta_1, \theta_2)}\left[\CR(\U\setminus\eta)^{-\mathfrak{r}}\one\{\CR(\U\setminus\eta)\le \eps\}\right]\notag\\
\le & N C^{(\mathfrak{r})}\prod_{k=2}^N H(\U; x_{a_k}, x_{b_k})^h \eps^{p-\mathfrak{r}}\Phi(\kappa, p; \sin^2((\theta_2-\theta_1)/4)),
\end{align*}
where we use~\eqref{eqn::CR_estimate2} to get the last inequality for any $0<\mathfrak{r}<p<1-\kappa/8$. 
\end{itemize}
Combining these two observations, we obtain~\eqref{eqn::asy_paired_aux2} and complete the proof. 
\end{proof}

\begin{lemma}\label{lem::asy_notpaired_right}
The asymptotic in~\eqref{eqn::multipleSLE_CR_pf_asynotpaired} with $j=1$ holds. 
\end{lemma}
\begin{proof}
In this case, we have $a_1=1, a_2=2<b_2<b_1$. 
The domain $\LC_{n}$ can be to the right of $\eta_1$ or to the left of $\eta_1$. We only prove the case when $\LC_{n}$ is to the right of $\eta_1$ and the other case can be proved similarly. 
We calculate the expectation conditional on $\eta_1$: 
\[\E_{\alpha}\left[\one\{0\in\LC_{n}\}\CR\left(\U\setminus\cup_{j=1}^N\eta_j\right)^{-\mathfrak{r}}\cond \eta_1\right]=
\frac{\LZ_{\alpha_1^R; n-1}^{(\mathfrak{r})}(\tilde{U}_1^R; x_2, \ldots, x_{b_1-1};0)}{\LZ_{\alpha_1^R}(U_1^R; x_2, \ldots, x_{b_1-1})},
\]
where $\LZ_{\alpha_1^R; n-1}^{(\mathfrak{r})}(\tilde{U}_1^R; x_2, \ldots, x_{b_1-1};0)$ is understood similarly as in~\eqref{eqn::asy_paired_aux1}. 
From Lemma~\ref{lem::multipleSLEvschordalSLE}, the law of $\eta_1$ under $\PP_{\alpha}$ is the same as $\eta\sim$ chordal $\SLE_{\kappa}$ in $(\U; x_1, x_{b_1})$ weighted by 
\begin{equation*}%\label{eqn::asy_notpaired_aux1}
\frac{\LZtwo(\U; x_1, x_{b_1})\LZ_{\alpha_1^R}(U_1^R; x_{2}, \ldots, x_{b_1-1})\LZ_{\alpha_1^L}(U_1^L; x_{b_1+1}, \ldots, x_{2N})}{\LZ_{\alpha}(\U; x_1, \ldots, x_{2N})}\one\{\LE_{\alpha}(\eta)\}.
\end{equation*}
Combining these two observations, we have
\begin{align*}
&\LZalpharn(\U; x_1, \ldots, x_{2N}; 0)\notag\\
=&\LZtwo(\U; x_1, x_{b_1})\E^{(\theta_1, \theta_{b_1})}\left[\LZ_{\alpha_1^R; n-1}^{(\mathfrak{r})}(\tilde{U}_1^R; x_2, \ldots, x_{b_1-1};0)\LZ_{\alpha_1^L}(U_1^L; x_{b_1+1}, \ldots, x_{2N})\one\{\LE_{\alpha}(\eta)\}\right]\\
\le &NC^{(\mathfrak{r})}\prod_{\{a,b\}\in\alpha}H(\U; x_a, x_b)^h\times \E^{(\theta_1, \theta_{b_1})}\left[\CR(\U\setminus\eta)^{-\mathfrak{r}}\one\{\LE_{\alpha}(\eta)\}\right],
\end{align*}
where we use~\eqref{eqn::multipleSLE_CRpf_upperbound_polygon}, \eqref{eqn::PPF_bound_polygon} and~\eqref{eqn::Poisson_mono} to get the inequality. To derive the conclusion, it suffices to show 
\begin{equation}\label{eqn::asy_notpaired_aux3}
\lim_{\theta_1, \theta_2\to\vartheta}(\theta_2-\theta_1)^{2h}\E^{(\theta_1, \theta_{b_1})}\left[\CR(\U\setminus\eta)^{-\mathfrak{r}}\one\{\LE_{\alpha}(\eta)\}\right]=0.
\end{equation}
There are two cases: Case 1. $h>0$, i.e. $\kappa\in (0,6)$; and Case 2. $h=0$, i.e. $\kappa=6$. 
\begin{itemize}
\item Case 1. $h>0$. Note that $(\theta_2-\theta_1)^{2h}\to 0$ as $\theta_1, \theta_2\to \vartheta$ and 
\begin{align*}
\E^{(\theta_1, \theta_{b_1})}\left[\CR(\U\setminus\eta)^{-\mathfrak{r}}\one\{\LE_{\alpha}(\eta)\}\right]\le& \E^{(\theta_1, \theta_{b_1})}\left[\CR(\U\setminus\eta)^{-\mathfrak{r}}\right]\\
=&\Phi(\kappa, \mathfrak{r}; \sin^2((\theta_{b_1}-\theta_1)/4))<\infty.
\end{align*}
This proves~\eqref{eqn::asy_notpaired_aux3} for $\kappa<6$. 
\item Case 2. $h=0$. Note that $\CR(\U\setminus\eta)^{-\mathfrak{r}}$ is integrable and $\PP^{(\theta_1, \theta_{b_1})}[\LE_{\alpha}(\eta)]\to 0$ as $\theta_1, \theta_2\to \vartheta$. Then bounded convergence theorem guarantees~\eqref{eqn::asy_notpaired_aux3} for $\kappa=6$. 
\end{itemize} 

\end{proof}
\begin{remark}\label{rem::solutionspace}
From Appendix~\ref{appendix::chordalBPZ}, the dimension of the solution space $\LS_N$ in~\eqref{eqn::chordaBPZ_space} of chordal BPZ equations is $N$:th Catalan number $C_N$. 
In the same spirit, we consider the solution space of the radial BPZ equations~\eqref{eqn::radialBPZ}. We fix $\kappa\in (0,6]$ and $\mathfrak{r}<1-\kappa/8$. We consider smooth functions defined on the configuration space 
\[\tilde{\chamber}_{2N}=\{(\theta_1, \ldots, \theta_{2N}): \theta_1<\theta_2<\cdots<\theta_{2N}<\theta_1+2\pi\}\]
subject to the following three conditions: radial BPZ equations~\eqref{eqn::radialBPZ}, rotation invariance, and power-law bound.
\begin{itemize}
\item \textnormal{\bf Rotation invariance:}
\begin{equation}\label{eqn::rotation_inv}
\LZ(\theta_1+\vartheta, \ldots, \theta_{2N}+\vartheta)=\LZ(\theta_1, \ldots, \theta_{2N}),
\end{equation} 
for all $\vartheta\in\R$.
\item \textnormal{\bf Power-law bound:}
There exist constants $C>0$ and $p>0$ such that for all 
$N \geq 1$ and $(\theta_1, \ldots, \theta_{2N}) \in \tilde{\chamber}_{2N}$, we have 
\begin{align}\label{eqn::radial_PLB_weak}
|\LZ(\theta_1, \ldots, \theta_{2N}) |\le 
C \prod_{1 \leq i<j \leq 2N}(\theta_j-\theta_i)^{\mu_{ij}(p)}, 
\quad \textnormal{where } \quad
\mu_{ij}(p) :=
\begin{cases}
p, \quad &\textnormal{if } |\theta_j-\theta_i| > 1, \\
-p, \quad &\textnormal{if } |\theta_j-\theta_i| < 1.
\end{cases}
\end{align}
\end{itemize} 
It is an interesting question to derive the dimension of the solution space 
\begin{equation}\label{eqn::radialBPZ_solutionspace}
\tilde{\LS}_N=\{F: \tilde{\chamber}_{2N}\to \C: F\text{ satisfies }~\eqref{eqn::radialBPZ}, \eqref{eqn::rotation_inv}, \eqref{eqn::radial_PLB_weak}\}.
\end{equation}

{\color{red}explain why they are linearly independent. This seems to be non-trivial?}

Propositions~\ref{prop::multipleSLE_CR_finite} and~\ref{prop::multipleSLE_CRpf_asy} give $(N+1)C_N$ linearly independent solutions for $\tilde{\LS}_N$, i.e. 
\[\dim(\tilde{\LS}_N)\ge (N+1)C_N.\]
We believe this lower bound is also the upper bound. 
See~\cite{WangWuCommutationRelation} for a detailed analysis for $N=1$. In particular,  \cite[Remark~3.13]{WangWuCommutationRelation} implies that $\dim(\tilde{\LS}_1)=2$.

More interestingly, there also exists a solution to radial BPZ equations~\eqref{eqn::radialBPZ} without~\eqref{eqn::rotation_inv} and~\eqref{eqn::radial_PLB_weak}. For $\mu\in\R$, the partition function for $2N$-sided radial $\SLE_{\kappa}$ with spiraling rate $\mu$
\begin{equation}
\LG_{\mu}(\theta_1, \ldots, \theta_{2N}):=\prod_{1\le i<j\le 2N}\left(\sin((\theta_j-\theta_i)/2)\right)^{2/\kappa}\times\exp\left(\frac{\mu}{\kappa}\sum_{j=1}^{2N}\theta_j\right)
\end{equation} 
also satisfies radial BPZ equations:
\begin{align}\label{eqn::radialBPZ_mu}
\frac{\kappa}{2}\frac{\partial_{j}^2\LZ}{\LZ}+\sum_{i\neq j}\left(\cot((\theta_i-\theta_j)/2)\frac{\partial_i\LZ}{\LZ}-\frac{(6-\kappa)/(4\kappa)}{\sin^2((\theta_i-\theta_j)/2)}\right)=\frac{\mu^2-3}{2\kappa},
\end{align}
for all $j\in\{1,\ldots, 2N\}$, see~\cite[Remark~3.9]{WangWuCommutationRelation}.  
\end{remark}



